Robust Asymmetric Loss for Multi-Label Long-Tailed Learning

In real medical data, training samples typically show long-tailed distributions with multiple labels. Class distribution of the medical data has a long-tailed shape, in which the incidence of different diseases is quite varied, and at the same time, it is not unusual for images taken from symptomatic patients to be multi-label diseases. Therefore, in this paper, we concurrently address these two issues by putting forth a robust asymmetric loss on the polynomial function. Since our loss tackles both long-tailed and multi-label classification problems simultaneously, it leads to a complex design of the loss function with a large number of hyper-parameters. Although a model can be highly fine-tuned due to a large number of hyper-parameters, it is difficult to optimize all hyper-parameters at the same time, and there might be a risk of overfitting a model. Therefore, we regularize the loss function using the Hill loss approach, which is beneficial to be less sensitive against the numerous hyper-parameters so that it reduces the risk of overfitting the model. For this reason, the proposed loss is a generic method that can be applied to most medical image classification tasks and does not make the training process more time-consuming. We demonstrate that the proposed robust asymmetric loss performs favorably against the long-tailed with multi-label medical image classification in addition to the various long-tailed single-label datasets. Notably, our method achieves Top-5 results on the CXR-LT dataset of the ICCV CVAMD 2023 competition. We opensource our implementation of the robust asymmetric loss in the public repository: https://github.com/kalelpark/RAL.

==> dummy.tex <==

% sota table to one column
% \begin{table*}[!t]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tblr}{
%   cells = {c},
%   cell{2}{1} = {r=8}{},
%   cell{2}{2} = {r=2}{},
%   cell{2}{8} = {r=8}{},
%   cell{2}{9} = {r=2}{},
%   cell{4}{2} = {r=2}{},
%   cell{4}{9} = {r=2}{},
%   cell{6}{2} = {r=2}{},
%   cell{6}{9} = {r=2}{},
%   cell{8}{2} = {r=2}{},
%   cell{8}{9} = {r=2}{},
%   hline{1-2} = {1,8}{l},
%   hline{1} = {1-6,,8-13}{1pt},
%   hline{1,10} = {6,13}{r},
%   hline{2} = {2-6,9-12}{},
%   hline{2} = {13}{r},
%   hline{10} = {1-6,8-13}{1pt},
% }
% Model                      & Method                       & Imagesize & mAP & mAUC & mF1 &  & Model    & Method     & Imagesize & mAP & mAUC & mF1 \\
% ResNet-50\cite{he2016deep} & CE                           & 224       & 0.222  & 0.736   & 0.159   &  & ConvNext-B\cite{liu2022convnet} & CE         & 224       & 0.301   & 0.808    & 0.218   \\
%                            &                              & 384       & 0.224  & 0.739   & 0.168   &  &          &            & 384       & 0.314   & 0.813    & 0.227   \\
%                            & Focal loss\cite{lin2017focal}& 224       & -   & -    & -   &  &          & Focal loss\cite{lin2017focal} & 224       & 0.304   & 0.807    & 0.231   \\
%                            &                              & 384       & -   & -    & -   &  &          &            & 384       & 0.295   & 0.803    & 0.224   \\
%                            & ASL\cite{ben2020asymmetric}  & 224       & -   & -    & -   &  &          & ASL\cite{ben2020asymmetric}        & 224       & 0.307   & 0.815    & 0.231   \\
%                            &                              & 384       & -   & -    & -   &  &          &            & 384       & 0.317   & 0.821    & 0.237   \\
%                            & Ours                         & 224       & -   & -    & -   &  &          & Ours       & 224       & 0.319   & 0.818    & 0.225   \\
%                            &                              & 384       & -   & -    & -   &  &          &            & 384       & 0.325   & 0.812    & 0.233   
% \end{tblr} }
% \caption{sota table}
% \label{tab:sota_table}
% \end{table*}

%-------------------------------------------------------------------------

%샘플1
% \begin{table}[]
% \small
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lll@{}}
% \toprule
% Methods    & Accuracy & F1-score \\ \midrule
% CE         & 0.850    & 0.716    \\
% Focal loss & 0.861    & 0.735    \\
% LDAM       & 0.849    & 0.728    \\
% OHEM       & 0.857    & 0.734    \\
% MTL        & 0.811    & 0.660    \\
% DANIL      & 0.825    & 0.667    \\
% CL         & 0.865    & 0.739    \\
% ProCo      & 0.887    & 0.763    \\
% Ours       & -        & -        \\ \bottomrule
% \end{tabular}%
% }
% \caption{ICIS2018 results}
% \label{tab:ICIS2018}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lll@{}}
% \toprule
% Methods    & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{F1-score} \\ \midrule
% CE         & 0.812                        & 0.608                        \\
% Focal loss & 0.815                        & 0.629                        \\
% LDAM       & 0.813                        & 0.620                        \\
% OHEM       & 0.813                        & 0.631                        \\
% MTL        & 0.813                        & 0.632                        \\
% DANIL      & 0.825                        & 0.660                        \\
% CL         & 0.825                        & 0.652                        \\
% ProCo      & 0.837                        & 0.674                        \\
% Ours       & -                            & -                            \\ \bottomrule
% \end{tabular}%
% }
% \caption{APTOS2019 results}
% \label{tab:APTOS2019}
% \end{table}

% Sample Tables

% %샘플2
% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tblr}{
%   cells = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {c=2}{},
%   cell{1}{4} = {c=2}{},
%   hline{1,12} = {-}{0.08em},
%   hline{2} = {2,3}{-}{0.05em},
%   hline{2} = {4}{l},
%   hline{2} = {4,5}{-}{0.05em},
%   hline{3} = {-}{0.05em},
% }
% Methods    & ICIS2018 &          & APTOS2019 &          \\
%            & Accuracy & F1-score & Accuracy  & F1-score \\
% CE         & 0.850    & 0.716    & 0.812     & 0.608    \\
% Focal loss\cite{lin2017focal} & 0.861    & 0.735    & 0.815     & 0.629    \\
% LDAM\cite{cao2019learning}       & 0.849    & 0.728    & 0.813     & 0.620    \\
% OHEM\cite{shrivastava2016training}       & 0.857    & 0.734    & 0.813     & 0.631    \\
% MTL\cite{liao2018deep}        & 0.811    & 0.660    & 0.813     & 0.632    \\
% DANIL\cite{gong2020distractor}      & 0.825    & 0.667    & 0.825     & 0.660    \\
% CL\cite{marrakchi2021fighting}         & 0.865    & 0.739    & 0.825     & 0.652    \\
% ProCo\cite{yang2022proco}      & 0.887    & 0.763    & 0.837     & 0.674    \\
% Ours       & -        & -        & -         & -        
% \end{tblr}
% }
% \caption{ICIS2018 \& APTOS2019 results}
% \label{tab:both}
% \end{table}


% \begin{table*}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}ccccccccccccc@{}}
% \cmidrule(r){1-6} \cmidrule(l){8-13}
% Model  & Method     & Imagesize & mAP & mAUC & mF1 &  & Model    & Method     & Imagesize & mAP & mAUC & mF1 \\ \cmidrule(r){1-6} \cmidrule(l){8-13} 
%        & CE         & 224       & -   & -    & -   &  &          & CE         & 224       & -   & -    & -   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & -   & -    & -   \\
%        & Focal loss & 224       & -   & -    & -   &  &          & Focal loss & 224       & -   & -    & -   \\
% ResNet &            & 384       & -   & -    & -   &  & ConvNexT &            & 384       & -   & -    & -   \\
%        & ASL        & 224       & -   & -    & -   &  &          & ASL        & 224       & -   & -    & -   \\ƒ
%        &            & 384       & -   & -    & -   &  &          &            & 384       & -   & -    & -   \\
%        & Ours       & 224       & -   & -    & -   &  &          & Ours       & 224       & -   & -    & -   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & -   & -    & -   \\ \cmidrule(r){1-6} \cmidrule(l){8-13} 
% \end{tabular}%
% }
% \caption{sota table}
% \label{tab:sota_table}
% \end{table*}

% Gaama : gamma_neg=4, gamma_pos=0, gamma_marign = 2.0, clip=0.05, eps = 0.02, margin = 1.0,

 % Gaama : gamma_neg=4, gamma_pos=0, gamma_marign = 2.0, clip=0.05, eps = 0.02, margin = 1.0,
% 본 Section에서는, 우리가 제안한 Enhanced Scarcity class aware Asymmetric Focal Loss를 ICCV 2023 CVAMD CXR-LT Dataset을 통하여 평가할 것입니다.  우리는 base를 AAA method를 위한 backbone model로 사용함. 모델을 학습할 때 이미지사이즈는 384로 학습했으며, augmentation으로는 resize, random flipping, random rotating, random sharpening, random erasing, gaussian blur를 적용했음. 네트워크의 optimizer는 adam을 사용했고 learning rate는 10-4로 설정했음. 효율적인 multi label classifiaction을 위해 \hyuk{Robust Asymmetric Focal
% Loss}를 사용했으며 batch size는 128로 설정했음. 모델은 총 6epoch동안 학습되었는데, 6epoch 이상 학습하면 \park{overfiiting하는 경향이 보였기 때문임. <-- 불필요 할 것 같습니다..! Formal하게 작성하는 것이 좋을 것 같습니당} 학습에는 RTX A5000 GPU를 8대 사용했으며 한번 학습 시 약 6시간 소요되었음


% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tblr}{
%   cells = {c},
%   cell{2}{1} = {r=8}{},
%   cell{2}{2} = {r=2}{},
%   cell{2}{8} = {r=8}{},
%   cell{2}{9} = {r=2}{},
%   cell{4}{2} = {r=2}{},
%   cell{4}{9} = {r=2}{},
%   cell{6}{2} = {r=2}{},
%   cell{6}{9} = {r=2}{},
%   cell{8}{2} = {r=2}{},
%   cell{8}{9} = {r=2}{},
%   hline{1-2} = {1,8}{l},
%   hline{1} = {2-5,,9-12}{},
%   hline{1,10} = {6,13}{r},
%   hline{2} = {2-6,9-12}{},
%   hline{2} = {13}{r},
%   hline{10} = {1-5,8-12}{},
% }

% Model  & Method     & Imagesize & mAP & mAUC & mF1 &  & Model    & Method     & Imagesize & mAP & mAUC & mF1 \\
% ResNet-50\cite{he2016deep} & CE         & 224       & 0.222  & 0.736   & 0.159   &  & ConvNext-B\cite{liu2022convnet} & CE         & 224       & 0.301   & 0.808    & 0.218   \\
%        &            & 384       & 0.224  & 0.739   & 0.168   &  &          &            & 384       & 0.314   & 0.813    & 0.227   \\
%        & Focal loss\cite{lin2017focal} & 224       & -   & -    & -   &  &          & Focal loss\cite{lin2017focal} & 224       & 0.304   & 0.807    & 0.231   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.295   & 0.803    & 0.224   \\
%        & ASL\cite{ben2020asymmetric}        & 224       & -   & -    & -   &  &          & ASL\cite{ben2020asymmetric}        & 224       & 0.307   & 0.815    & 0.231   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.317   & 0.821    & 0.237   \\
%        & Ours       & 224       & -   & -    & -   &  &          & Ours       & 224       & -   & -    & -   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.325   & 0.822    & 0.294   
% \end{tblr}}
% \caption{sota table}
% \label{tab:sota_table}
% \end{table*}

% \hyuk{저희 주제가 loss라서 loss끼리만 비교하는것도 좋을거같습니다. multi label뿐만 아니라 single label에서도 잘 동작한다는것을 보여주는 목적으로요. long tailed dataset에서 다른 loss보다 성능이 높게 나왔습니다. 특히 APTOS는 acc, f1 둘 다 높았고, ISIC는 acc는 좀 떨어지지만 f1은 제일 높게 나왔습니다. long tailed엔 f1이 더 효과적인 성능지표라는것을 강조해야할거같아요. asl은 직접 학습시킨 결과입니다}


% \begin{table}[!h]
% \centering
% \resizebox{\columnwidth}{!}
%     {
%     \begin{tblr}{
%           cells = {c},
%           cell{1}{1} = {r=2}{},
%           cell{1}{2} = {c=2}{},
%           cell{1}{4} = {c=2}{},
%           hline{1,12} = {-}{0.08em},
%           hline{2} = {2,3}{-}{0.05em},
%           hline{2} = {4}{l},
%           hline{2} = {4,5}{-}{0.05em},
%           hline{3} = {-}{0.05em},
%           hline{8} = {-}{0.08em},
%         }
%         Methods    & ICIS2018 &          & APTOS2019 &          \\
%                    & Accuracy & F1-score & Accuracy  & F1-score \\
%         CE         & 0.850    & 0.716    & 0.812     & 0.608    \\
%         Focal loss\cite{lin2017focal} & \textbf{0.861}    & 0.735    & 0.815     & 0.629    \\
%         LDAM\cite{cao2019learning}       & 0.849    & 0.728    & 0.813     & 0.620    \\
%         Asl loss\cite{ben2020asymmetric}       & 0.854    & 0.734    & 0.840     & 0.680    \\
%         \textbf{royal loss (ours)}       & 0.852        & \textbf{0.740}        & \textbf{0.845} & \textbf{0.694}        
%         \end{tblr} 
%     }
% \caption{ICIS2018 \& APTOS2019 results }
% \label{tab:both}
% \end{table}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tblr}{
%   cells = {c},
%   cell{2}{1} = {r=8}{},
%   cell{2}{2} = {r=2}{},
%   cell{2}{8} = {r=8}{},
%   cell{2}{9} = {r=2}{},
%   cell{4}{2} = {r=2}{},
%   cell{4}{9} = {r=2}{},
%   cell{6}{2} = {r=2}{},
%   cell{6}{9} = {r=2}{},
%   cell{8}{2} = {r=2}{},
%   cell{8}{9} = {r=2}{},
%   hline{1-2} = {1,8}{l},
%   hline{1} = {2-5,,9-12}{},
%   hline{1,10} = {6,13}{r},
%   hline{2} = {2-6,9-12}{},
%   hline{2} = {13}{r},
%   hline{10} = {1-5,8-12}{},
% }

% Model  & Method     & Imagesize & mAP & mAUC & mF1 &  & Model    & Method     & Imagesize & mAP & mAUC & mF1 \\
% ResNet-50\cite{he2016deep} & CE         & 224       & 0.222  & 0.736   & 0.159   &  & ConvNext-B\cite{liu2022convnet} & CE         & 224       & 0.301   & 0.808    & 0.218   \\
%        &            & 384       & 0.224  & 0.739   & 0.168   &  &          &            & 384       & 0.314   & 0.813    & 0.227   \\
%        & Focal loss\cite{lin2017focal} & 224       & -   & -    & -   &  &          & Focal loss\cite{lin2017focal} & 224       & 0.304   & 0.807    & 0.231   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.295   & 0.803    & 0.224   \\
%        & ASL\cite{ben2020asymmetric}        & 224       & -   & -    & -   &  &          & ASL\cite{ben2020asymmetric}        & 224       & 0.307   & 0.815    & 0.231   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.317   & 0.821    & 0.237   \\
%        & Ours       & 224       & -   & -    & -   &  &          & Ours       & 224       & -   & -    & -   \\
%        &            & 384       & -   & -    & -   &  &          &            & 384       & 0.325   & 0.822    & 0.294   
% \end{tblr}}
% \caption{sota table}
% \label{tab:sota_table}
% \end{table*}

% \begin{table}[!h]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule    
%             Focal Loss & Asymmetric &   Weight & Ours &mAP & mAUC   \\ \hline
%             \checkmark &            &          &      &0.295 & 0.803   \\ 
%             \checkmark & \checkmark &          &      &0.317 & 0.811   \\
%             \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & &0.319 & \textbf{0.818}  \\ 
%             \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} &\textbf{\checkmark} &\textbf{0.323} & 0.817  \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Component of Ours}
%     \label{tab:component_table}
% \end{table}

% \begin{figure}[!ht]%
%     \begin{minipage}{\columnwidth}
%     \begin{minipage}][b]{0.49\columnwidth}
%         \centering
%         \includegraphics[width=0.5\columnwidth, height=4.2cm]
%         \captionof{figure}{Compare of $alpha$ parameter with APL}
%     \subfloat[\centering Compare of $\alpha$ parameter with APL]{{{Imgs/epsilon_neg_test.pdf} }}%
%     % \qquad
%     \subfloat[\centering Compare of $\lambda$ parameter]{{\includegraphics[width=0.5\columnwidth, height=4.2cm]{Imgs/lambda_test.pdf} }}%
%     \caption{Effective of parameter. To understand the performace about forcus parameter and weight term parameter, (a)에서는 우리의 방식과 APL에서 사용되는 forcus parameter $\alpha$를 조정한 결과를 나타냄. 우리의 방식은 APL보다 약 1\%높은 AUC를 달성하였으며 $\alpha$값에 관계없이 일반적인 성능을 보여주는 것을 확인할 수 있음. (b)에서는 Re-weight parameter $\lambda$의 값을 조정한 결과를 나타내며 $\lambda = 2.5$일때 가장좋은 AUC 성능을 달성하는 것을 확인하였음. \hyuk{legend 위치 통일하면 좋을거같아요}
%     \ryu{b에 APL없음.} 
%     }%
%     \label{fig:hyperparameter}%
% \end{figure}



% \begin{figure}[!t]
% \includegraphics[width=0.8\columnwidth, height=5cm]{Imgs/epsilon_neg_test.pdf}
% \caption{Compare of $alpha$ paramter with APL.}
% \label{fig:noise_image}
% \end{figure}



% \begin{table*}[!t]
% \centering
% \begin{threeparttable}
% \setlength{\tabcolsep}{10pt}
%     \begin{tabular}{cccccc}
%     \toprule
%     Label                  & Positive(\%) & Negative(\%)      & Label                  & Positive(\%) & Negative(\%) \\ \hline
%     Atelectasis                &  67.6(0.26)  & 197.2(0.74)                & Mass                   &  5.6(0.02)   & 259.3(0.98)    \\
%     Calcification              &  43.7(0.02)   & 26.0(0.98)                & No Finding             &  41.9(0.16)  & 22.3(0.84)     \\
%     Cardiomegaly               &  76.9(0.29)  & 188.0(0.71)                & Nodule                 &  76.7(0.03)   & 257.2(0.97)      \\
%     Consolidation              & 16.0(0.06)  & 248.8(0.94)               & Pleural Effusion       &  69.2(0.26)  & 195.7(0.74)     \\
%     Edema                      & 38.6(0.15)  & 226.3(0.85)              & Pleural Other          &  0.7(0.0)     & 264.2(1.0)   \\
%     Emphysema                  &   4.3(0.02)   & 260.6(0.98)             & Pleural Thickening     &  3.7(0.01)   & 261.4(0.99)     \\
%     Cardiomediastinum          & 30.1(0.11)  & 234.8(0.89)              & Pneumomediastinum      & 0.8(0.0)     & 264.0(1.0)       \\
%     Fibrosis                   &  1.2(0.0)    & 263.7(1.0)              & Pneumonia              &  48.1(0.18)  & 216.8(0.82)   \\
%     Fracture                   & 11.9(0.04)  & 252.9(0.96)             & Pneumoperitoneum       &  0.5(0.0)     & 264.3(1.0)    \\
%     Hernia                     & 0.4(0.02)   & 260.8(0.98)             & Pneumothorax           &  14.9(0.06)  & 249.9(0.94)   \\
%     Infiltration               &  10.2(0.04)  & 254.6(0.96)              & Emphysema              & 0.2(0.01)   & 262.3(0.99)   \\
%     Lung Lesion                &  2.5(0.01)   & 262.3(0.99)               & Support Devices        &89.1(0.34)  & 175.7(0.66)    \\
%     Lung Opacity               &   79.9(0.3)   & 184.9(0.7)             & Tortuous Aorta         &  3.4(0.01)   & 261.3(0.99)     \\ \bottomrule
%     \multicolumn{6}{r}{Note: Values are in 'K' 
%     (thousands)} 
%     \end{tabular}
%     \caption{Specification of the CXR-LT dataset. It shows that the samples are heavily distributed in a few classes while several classes have very few samples.
%     }
%     \label{tab:descript_dataset}
%      \end{threeparttable}
% \end{table*}


%\begin{table*}[!t]
%\centering
%\setlength{\tabcolsep}{10pt}
%    \begin{tabular}{cccccc}
%    \toprule
%    Label                  & Positive(\%) & Negative(\%)      & Label                  & Positive(\%) & Negative(\%) \\ \hline
%    Atelectasis                &  67597(0.26)  & 197252(0.74)                & Mass                   &  5529(0.02)   & 259320(0.98)    \\
%    Calcification              &  4361(0.02)   & 260488(0.98)                & No Finding             &  41869(0.16)  & 222980(0.84)     \\
%    Cardiomegaly               &  76900(0.29)  & 187949(0.71)                & Nodule                 &  7663(0.03)   & 257186(0.97)      \\
%    Consolidation              & 16038(0.06)  & 248811(0.94)               & Pleural Effusion       &  69240(0.26)  & 195609(0.74)     \\
%    Edema                      & 38574(0.15)  & 226275(0.85)              & Pleural Other          &  675(0.0)     & 264174(1.0)   \\
%    Emphysema                  &   4255(0.02)   & 260594(0.98)             & Pleural Thickening     &  3369(0.01)   & 261480(0.99)     \\
%    Cardiomediastinum          & 30119(0.11)  & 234730(0.89)              & Pneumomediastinum      & 788(0.0)     & 264061(1.0)       \\
%    Fibrosis                   &  1158(0.0)    & 263691(1.0)              & Pneumonia              &  48093(0.18)  & 216756(0.82)   \\
%    Fracture                   & 11883(0.04)  & 252966(0.96)             & Pneumoperitoneum       &  543(0.0)     & 264306(1.0)    \\
%    Hernia                     & 4049(0.02)   & 260800(0.98)             & Pneumothorax           &  14983(0.06)  & 249866(0.94)   \\
%    Infiltration               &  10218(0.04)  & 254631(0.96)              & Emphysema              & 2453(0.01)   & 262396(0.99)   \\
%    Lung Lesion                &  2533(0.01)   & 262316(0.99)               & Support Devices        &89140(0.34)  & 175709(0.66)    \\
%    Lung Opacity               &   79931(0.3)   & 184918(0.7)             & Tortuous Aorta         &  3499(0.01)   & 261350(0.99)     \\ \bottomrule
%    \end{tabular}
%    \caption{Detail description of MIMIC-CXR-LT daataset.
%    \ryu{67597을 67.6으로 하고 단위를 K라고 명시할 것.}
%    }
%    \label{tab:descript_dataset}
%\end{table*}
